Towards Accurate and Efficient 3D Object Detection for Autonomous Driving: A Mixture of Experts Computing System on Edge

This paper presents Edge-based Mixture of Experts (MoE) Collaborative Computing (EMC2), an optimal computing system designed for autonomous vehicles (AVs) that simultaneously achieves low-latency and high-accuracy 3D object detection. Unlike conventional approaches, EMC2 incorporates a scenario-aware MoE architecture specifically optimized for edge platforms. By effectively fusing LiDAR and camera data, the system leverages the complementary strengths of sparse 3D point clouds and dense 2D images to generate robust multimodal representations. To enable this, EMC2 employs an adaptive multimodal data bridge that performs multi-scale preprocessing on sensor inputs, followed by a scenario-aware routing mechanism that dynamically dispatches features to dedicated expert models based on object visibility and distance. In addition, EMC2 integrates joint hardware-software optimizations, including hardware resource utilization optimization and computational graph simplification, to ensure efficient and real-time inference on resource-constrained edge devices. Experiments on open-source benchmarks clearly show the EMC2 advancements as an end-to-end system. On the KITTI dataset, it achieves an average accuracy improvement of 3.58% and a 159.06% inference speedup compared to 15 baseline methods on Jetson platforms, with similar performance gains on the nuScenes dataset, highlighting its capability to advance reliable, real-time 3D object detection tasks for AVs. The official implementation is available at https://github.com/LinshenLiu622/EMC2.

==> sec/5_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

Our current work primarily focuses on optimizing the algorithmic framework and deployment module. To achieve a more comprehensive solution for the algorithm, software, and hardware co-optimization work, we will explore topics related to dataset augmentation and hardware management. These advancements are expected to further enhance system robustness, efficiency, and adaptability in real-world applications.

In terms of dataset expansion, we plan to leverage large language models (LLMs)~\citep{kasneci2023chatgpt} and other generative AI techniques~\citep{fui2023generative} to synthesize additional edge-case data. Such data augmentation will enable the model to better generalize across diverse and challenging scenarios, reducing algorithmic constraints and improving overall performance. By generating synthetic yet realistic training samples, we aim to mitigate data scarcity issues, enhance robustness to out-of-distribution cases, and lower the reliance on costly real-world data collection. Furthermore, we will explore self-supervised learning strategies to maximize the utility of both synthetic and real-world datasets while minimizing manual annotation efforts.

For hardware management, we will incorporate state-of-the-art load-balancing techniques, such as~\citep{dai2018joint} and~\citep{zhang2019task}, to dynamically allocate computational resources across different threads at varying time intervals. This dynamic resource scheduling will optimize hardware utilization, minimize latency, and ensure efficient workload distribution. This technique will investigate adaptive resource management strategies that leverage real-time performance monitoring and predictive modeling to allocate computing power more effectively. These strategies will allow the system to respond dynamically to variations in computational demand, thereby achieving optimal trade-offs between energy consumption and processing speed.

Moreover, we intend to integrate these optimizations into a scalable and modular architecture, facilitating seamless deployment across diverse hardware platforms. By further bridging the gap between software and hardware optimization, we aspire to create a more efficient, adaptive, and high-performance system capable of addressing the evolving demands of real-world applications.

==> sec/Relatedwork_extension.tex <==
%\section{Related Work Extension}

%\textbf{Apple-to-apple Object Detection Algorithm Comparison.} To better illustrate runtime performance on edge, we tested several common algorithms on the Nvidia Jetson platform, with accuracy and latency results shown in Tab.~\ref{tab:comparison}. The KITTI~\citep{andreas2012kitti} dataset sets sampled objects into three levels based on the number of pixels: Easy, Moderate, and Hard. To ensure high precision and low latency across all difficulty levels, we integrate the low-latency advantage of LiDAR-only models with the high precision of LiDAR-plus-RGB models using the MoE-based framework $\mathrm{EMC2}$, which dynamically selects experts based on each scenario, as detailed in Sec.~\ref{sec:sad}. A high-level comparison of $\mathrm{EMC2}$ characteristics with existing end-to-end SOTA detection systems is presented in Tab.~\ref{tab:related work comparison}.

\begin{table}[htbp]
\footnotesize
\setlength{\tabcolsep}{3pt}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccc}
\Xhline{1.2pt}
\multirow{3}{*}{\textbf{Method}}  & \multicolumn{2}{c}{\rule{0pt}{1.1em}\textbf{Easy}} & \multicolumn{2}{c}{\textbf{ Moderate}} & \multicolumn{2}{c}{\textbf{Hard}}  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
  & \textbf{Acc.} & \textbf{Latency} & \textbf{Acc.} & \textbf{Latency} & \textbf{Acc.} & \textbf{Latency}  \\
\midrule
RGB  &\cellcolor{blue!20} \cmark\cellcolor{blue!20} \cmark&  \xmark & \cellcolor{blue!10} \cmark&  \xmark & \xmark &  \xmark &    \\ 
LiDAR  & \cellcolor{blue!20} \cmark\cellcolor{blue!20} \cmark&  \cellcolor{blue!10} \cmark&\cellcolor{blue!10} \cmark& \cellcolor{blue!10} \cmark & \xmark & \cellcolor{blue!10} \cmark& \\
LiDAR+RGB  & \cellcolor{blue!20} \cmark\cellcolor{blue!20} \cmark& \xmark  &\cellcolor{blue!20} \cmark\cellcolor{blue!20}\cmark&  \xmark &\cellcolor{blue!20} \cmark\cellcolor{blue!20}\cmark&  \xmark  &  \\
$\mathrm{EMC2}$ \textbf{(Ours)}  &  \cellcolor{blue!20} \cmark\cellcolor{blue!20} \cmark&  \cellcolor{blue!10} \cmark&  \cellcolor{blue!20} \cmark\cellcolor{blue!20} \cmark&  \cellcolor{blue!10} \cmark&  \cellcolor{blue!20} \cmark\cellcolor{blue!20} \cmark&  \cellcolor{blue!10} \cmark&  \\
\Xhline{1.2pt}
\end{tabular}}
\vspace{-0.1in}
\caption{\textbf{Comparison of existing end-to-end detection system with EMC2.} A double checkmark denotes average precision AP over 80\%, a single checkmark for AP 70\%–80\%, and a checkmark for latency under 400 ms on edge device Nvidia Jetson.}
\label{tab:related work comparison}
\end{table}

\section{Method Extension}
\subsection{Algorithm for Multimodal Fusion}
Alg.~\ref{alg:fusion} presents the pseudocode for multimodal fusion of LiDAR and image data, where LiDAR voxel features are combined with image features projected into 3D space, as discussed in Sec.~\ref{sec:amdb} and Sec.~\ref{sec:experts}. Specifically, pixels aligned with a voxel in 3D space have their image features concatenated with the voxel’s LiDAR features, while others are concatenated with zero-filled features. However, this fusion process is memory-intensive, posing challenges for edge computing devices. To address this, our Hierarchical Training and Multiscale Pooling are jointly designed to optimize memory usage and computational efficiency.

\begin{algorithm}
\caption{Fusion of Image Features into 3D Space}
\label{alg:fusion}
\begin{algorithmic}[1] % 开启行号
\Require Features and 3D coordinates of LiDAR voxels $\mathcal{V}=\{f_{v_i}, v_i\}_{i=1}^N$, Features and 3D coordinates of image pixels $\mathcal{P}=\{f_{p_j}, p_j\}_{j=1}^M$, Proposal regions derived from LiDAR data $\mathcal{R}=\{r_k\}_{k=1}^K$

\Ensure Fused multimodal features $\mathcal{V}^\text{fused}$

\State Initialize $\mathcal{V}^\text{fused} = \{v_i^\text{fused} \mid v_i^\text{fused} = [f_{v_i}, 0], \forall v_i \in \mathcal{V}\}$
\For{$r_k \in \mathcal{R}$}
    \State Identify pixels $\mathcal{P}_k = \{p_j \mid p_j \in r_k\}$
    \For{$p_j \in \mathcal{P}_k$}
        % \State Compute the voxel index $i$ corresponding to $p_j$'s 3D coordinate
        \If{$p_j$ exists in $\mathcal{V}$}
            \State $v_i^\text{fused} \gets [f_{v_i}, f_{p_j}]$
        \Else
            % \State $v_i^\text{fused} \gets [0, f_{p_j}]$ \\
            \State $\mathcal{V}^\text{fused} \gets \mathcal{V}^\text{fused} \cup \{[0, f_{p_j}]\}$
        \EndIf
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Optimized 3D Sparse Convolution Algorithm}
3D sparse convolution has a computational complexity of $O(\mathcal{N}\times \mathcal{C}_{\text{in}}\times \mathcal{K}^3\times \mathcal{C}_{\text{out}})$, whereas dense convolutions operate at $O(\mathcal{H}^3\times \mathcal{C}_{\text{in}}\times \mathcal{K}^3\times \mathcal{C}_{\text{out}})$, where $\mathcal{H}^3$ represents the total spatial domain, $\mathcal{N}$ represents the number of nonzero voxels, $\mathcal{C}_{\text{in}}$ and $\mathcal{C}_{\text{out}}$ denote the input and output channels, and $\mathcal{K}^3$ represents the kernel size. By restricting computation to nonzero voxels, sparse convolution significantly reduces redundant operations, thereby improving efficiency and lowering computational overhead by $65$–$80\%$~\cite{yan2018second}, making it well-suited for resource-constrained environments.

Alg.~\ref{alg:spconv} presents the pseudocode of our customized 3D sparse convolution operator under ONNX Runtime. Specifically, the non-empty voxel index search within the sparse tensor is optimized using prefix scanning. Moreover, the \textit{Fused Multiply-Add} (FMA) operation, which serves as the core convolution operation, leverages parallel communication and computation, as well as computation graph refinement through operator node fusion. These edge-oriented system-level optimizations are detailed in Sec.~\ref{sec:sysOpt}.

\begin{algorithm}
\caption{Optimized Sparse 3D Convolution}
\label{alg:spconv}
\begin{algorithmic}[1]
\Require Input non-empty voxels $\mathcal{V}_{\mathrm{in}}=\{f_{\mathrm{in}}^i, o_{\mathrm{in}}^i\}_{i=1}^N$, where $f$ is input features and $o$ is input voxel coordinates; Convolution kernel $\mathcal{K}$; Voxel Space $\mathcal{H}$.

\Ensure Output non-empty voxels $\mathcal{V}_{\mathrm{out}}=\{f_{\mathrm{out}}^i, o_{\mathrm{out}}^i\}_{i=1}^N$.

\For {$v_{\mathrm{in}}^i = \{f_{\mathrm{in}}^i, o_{\mathrm{in}}^i\} \in \mathcal{V}_{\mathrm{in}}$} \textbf{in parallel}
    \State $(\mathrm{x}_{k_0}, \mathrm{y}_{k_0}, \mathrm{z}_{k_0}) \gets o_{\mathrm{in}}^i$\;\textcolor{gray}{\textit{\# Align kernel center to voxel}}
\State \textcolor{gray}{\textit{\# Collect all voxels currently covered by kernel}}
\State $\mathcal{V}_{\mathrm{part}} \gets \emptyset$
    \For {$v^j_{\text{in}}=\{f_{\mathrm{in}}^j, o_{\mathrm{in}}^j\}$}
        \For{$(\mathrm{x}_{k}, \mathrm{y}_{k}, \mathrm{z}_{k}) \in \mathcal{K}$} 
            \State $o_{\mathrm{neighbor}} \gets (\mathrm{x}_{k_0} + \mathrm{x}_{k}, \mathrm{y}_{k_0} + \mathrm{y}_{k}, \mathrm{z}_{k_0} + \mathrm{z}_{k})$
            
            \If{$o_{\mathrm{neighbor}} \in \mathcal{V}_{\mathrm{in}}$ \textbf{and} $o_{\mathrm{neighbor}} \in \mathcal{H}$}
                \State $\mathcal{V}_{\mathrm{part}} \gets \mathcal{V}_{\mathrm{part}} \cup \{(f_{\mathrm{in}}^j, o_{\mathrm{neighbor}})\}$
            \EndIf
        \EndFor
    \EndFor
\State \textcolor{gray}{\textit{\# Fused Multiply-Add (FMA) as convolution}}
\State $(f_{\mathrm{out}}^i, o_{\mathrm{out}}^i) \gets \mathbf{FMA}(\mathcal{V}_{\mathrm{part}}, \mathcal{K})$
\EndFor
\end{algorithmic}
\end{algorithm}


\subsection{Memory Optimization Elaboration}
\textbf{Streaming Multiprocessor (SM) and Shared Memory.} As shown in Fig.~\ref{fig:cores}, SMs are the core computational units of a GPU, each containing multiple cores for parallel execution. When a kernel is launched, it defines computation blocks that are distributed across SMs. Shared memory is a high-speed cache within each SM, reducing global memory access by enabling data sharing among cores. It facilitates communication between threads within a block, improving data exchange efficiency by reducing global memory access. Optimizing its usage significantly boosts GPU performance. To leverage this, the ONNX compiler is configured to maximize shared memory utilization and optimize execution order across warps, minimizing redundant memory access and ultimately enhancing computational efficiency.

\textbf{Parallel Communication and Computation.} Parallel communication and computation are essential for memory optimization. A naive approach would load all data to the GPU before any computation begins, restricting the GPU to either computation or communication at a given time. To fully utilize GPU resources, matrices are partitioned into multiple chunks. While some chunks are being processed, the next chunk is loaded into memory, and the previous chunk is offloaded, enabling concurrent computation and communication to improve efficiency. The process operates as follows: 1) The host dispatches a kernel to the GPU, defining a computational task; 2) The scheduler assigns block $0$ to an SM, reserving execution contexts and shared memory; 3) Remaining blocks are assigned to available execution units in an interleaved manner; 4) Once block $0$ completes execution, block $4$ is assigned to the freed core, and the process repeats. This procedure is illustrated in Fig.~\ref{fig:cores}.

\section{Result Visualization}
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{vis.pdf}
    \caption{\textbf{Visualization of detection result of two baselines and our approach.} We select four representative scenarios: (a) intersection, (b) standard, (c) narrow street, and (d) dense surrounding. The first two rows show the detection results of PV-RCNN~\citep{shi2020pv} and SECOND~\citep{yan2018second}, respectively. The third row illustrates the proposal regions generated by our \textit{AMDB}, while the fourth row presents the final detection results of $\mathrm{EMC2}$. Spherical markers highlight voxels within bounding boxes. In the last two rows representing our model, darker spheres indicate voxels with higher confidence scores, while lighter spheres correspond to lower confidence scores. In contrast, the spheres in the first two rows (baselines) are colored solely for visualization purposes. Compared to the two baselines, $\mathrm{EMC2}$ significantly reduces both false positive and false negative detections.}
\label{fig:vis}
\end{figure*}
Fig.~\ref{fig:vis} presents the detection results of PV-RCNN~\citep{shi2020pv} and Second~\citep{yan2018second} as baselines, alongside with our intermediate (output of \textit{AMDB}) and final results, on four representative scenes from the KITTI validation dataset.

For objects closer to the LiDAR sensor, stronger reflection intensity results in a higher number of valid voxels and higher confidence scores. As distance increases, reflection weakens~\citep{reymann2015improving}, LiDAR points become sparser, and confidence scores decline. 

For vehicles, reflections from windows and rooftops fade the fastest, disappearing beyond $60$ meters, while signals from doors weaken gradually and vanish after $90$ meters. The vehicle body and tire framework remain detectable within 120 meters but disappear beyond this range~\citep{reymann2015improving}. Vehicles moving in the opposite direction tend to have lower scores for windows and rooftops due to smaller LiDAR reflection angles. Pedestrians and bicycles exhibit more variability. At the same distance, confidence scores of voxels for pedestrians can differ significantly, largely due to variations in clothing materials~\citep{reymann2015improving}. In contrast, bicycles generally maintain consistent confidence scores across different parts at the same distance, though all scores decline uniformly with increasing distance. 

Regarding occlusion, since the LiDAR sensor is roof-mounted~\citep{liu2019should}, it acquires rich information from vehicles in the same lane. As shown in Fig.~\ref{fig:vis}, pedestrians, vehicles, and bicycles can be robustly detected because their LiDAR signals exhibit significant differences in height and spatial distribution compared to background points. This enables 3D sparse convolution to extract spatial features like distance and height, despite interference from ground clutter.

Compared to $\mathrm{EMC2}$, PV-RCNN~\citep{shi2020pvrcnn} exhibits one additional false positive and one false negative for pedestrians in scenario (a), as well as one false negative and three false positives for cars. In scenario (b), it introduces one additional false positive for cars. In scenario (c), although it has two fewer false positives for cars, it produces four additional false negatives for pedestrians. In scenario (d), there are two additional false positives for pedestrians. Similarly, in comparison to $\mathrm{EMC2}$, Second~\citep{yan2018second} generates two extra false positives for both cars and pedestrians in scene (a). In scene (b), it adds three false positives for each of bicycles, pedestrians, and cars. In scenario (c), it produces three more false positives for cars, one for pedestrians, and three for bicycles. In scenario (d), it has two fewer false negatives for pedestrians but introduces three additional false positives for cars and one more for pedestrians.


\clearpage
\setcounter{page}{1}
% \maketitlesupplementary

\setcounter{section}{0} % let the section starts from A 
\renewcommand{\thesection}{\Alph{section}} 

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{cores.pdf}
    \caption{\textbf{Illustration of Streaming Multiprocessor (SM), Shared Memory, and Parallel Communication and Computation.} }
    \label{fig:cores}
    \vspace{-4mm}
\end{figure*}
